Augment with Care: Contrastive Learning for Combinatorial Problems

Supervised learning can improve the design of state-of-the-art solvers for combinatorial problems, but labelling large numbers of combinatorial instances is often impractical due to exponential worst-case complexity. Inspired by the recent success of contrastive pre-training for images, we conduct a scientific study of the effect of augmentation design on contrastive pre-training for the Boolean satisfiability problem. While typical graph contrastive pre-training uses label-agnostic augmentations, our key insight is that many combinatorial problems have well-studied invariances, which allow for the design of label-preserving augmentations. We find that label-preserving augmentations are critical for the success of contrastive pre-training. We show that our representations are able to achieve comparable test accuracy to fully-supervised learning while using only 1% of the labels. We also demonstrate that our representations are more transferable to larger problems from unseen domains. Our code is available at https://github.com/h4duan/contrastive-sat.

==> body/method_arxiv.tex <==
\section{Framework Overview}


\begin{figure*}[th]
    \centering
    \begin{tikzpicture}
    \node at (0,0) {\includegraphics[width=2\columnwidth]{body/fig/framework.pdf}};
    
    % \tikzstyle{nome}=[anchor=west]
    
    \scriptsize
    \draw (-7.4, 0.4)  node[right] {$c_1:x_1$};
    \draw (-7.4, 0.4 - 0.35)  node[right] {$c_2: x_2 \lor x_3 $};
    \draw (-7.4, 0.4 - 2 * 0.35)  node[right] {$c_3: x_1 \lor \neg x_3 \lor x_4 $};
    \draw (-7.4, 0.4 - 3 * 0.35)  node[right] {$c_4: \neg x_1 \lor x_2 \lor x_3 \lor \neg x_4$};
    
    \draw (-2.8, 1.45)   node[right] {\st{$c_1: x_1$}};
    \draw (-2.8, 1.45  - 0.35)  node[right] {$c_2: x_2 \lor x_3$};
    \draw (-2.8, 1.45  - 2 * 0.35) node[right] {\st{$c_3: x_1 \lor \neg x_3 \lor x_4 $}};
    \draw (-2.8, 1.45  - 3 * 0.35)  node[right] {$c_4\!\!: $\st{$\neg x_1 \lor$} $ x_2 \lor x_3 \lor \neg x_4$};
    
    \draw (-2.8, -0.55)   node[right] {$c_1: x_1$};
    \draw (-2.8, -0.55 - 0.35)  node[right] {\st{$c_2: x_2 \lor x_3$}};
    \draw (-2.8, -0.55 - 2 * 0.35)  node[right] {\st{$c_3: x_1 \lor \neg x_3 \lor x_4 $}};
    \draw (-2.8, -0.55 - 3 * 0.35)   node[right] {\st{$c_4: \neg x_1 \lor x_2 \lor x_3 \lor \neg x_4$}};
    \draw (-2.8, -0.55 - 4 * 0.35)   node[right] {\color{our_red} $c_5: x_1 \lor x_2 \lor x_4$};
    
    
    \footnotesize
    \draw (-5.3, 2.)   node[left] {Label};
    \draw (-5.3, 1.65)  node[left] {Preserving};
     \draw (-5.3, 1.35)  node[left] {Augmentations};
    
    \normalsize
    \draw (5.8, 0.55) node {Encoder};
    \draw (5.8, -1.4) node {Encoder};
    
    \draw (2.5, 0.55) node {$G_1$};
    \draw (2.5, -1.7) node {$G_2$};
    
    \draw (1.2, 0.65)   node {$\mathcal{E}$};
    \draw (1.2, -1.45)   node {$\mathcal{E}$};
    
    \draw (6.8, 0)   node {$\mathbf{z_1}$};
    \draw (6.8, -1.95)   node {$\mathbf{z_2}$};
    
    \large
    \draw (-6.0, -1.1)   node {$\phi$};
    \draw (-1.2, -0.1)   node {$\hat{\phi}_1$};
    \draw (-1.2, -2.4)  node {$\hat{\phi}_2$};
    
    \Large
    \draw (7.8, -0.25)   node {$\mathcal{L(.)}$};
    
 \end{tikzpicture}
    \caption{Our contrastive learning framework for combinatorial problems. Given an instance $\phi$, a pair of augmented samples $(\hat{\phi}_1$, $\hat{\phi}_2)$ are formed using label-preserving augmentations. $(\hat{\phi}_1$, $\hat{\phi}_2)$ are then transformed to graph formats $(G_1, G_2)$. An encoder is used to extract graph representations $(\mathbf{z}_1, \mathbf{z}_2)$. Lastly, a standard contrastive loss is applied over a mini-batch of instances.} 
     \label{fig:cocl_model}
\end{figure*}

Similar to contrastive algorithms in other domains (e.g., images), we learn representations by contrasting augmented views of the same instance against negative samples. Our framework (Figure \ref{fig:cocl_model}) consists of four major components:
    
    \textbf{Augmentations.}
    Given a combinatorial instance $\phi$, a stochastic augmentation is applied to form a pair of positive samples, denoted by $(\hat{\phi}_1$, $\hat{\phi}_2)$. Our key insight is the tailored design of augmentations for combinatorial problems should preserve the label of the problem, e.g., satisfiability for SAT, as detailed in Section \ref{sec: lpa}. 
    
    
    
    \textbf{Format Transformation ($\mathcal{E}$).}
    Formulas $(\hat{\phi}_1$, $\hat{\phi}_2)$ are transformed into (e.g., $\text{LIG}^{+}$) graphs $(G_1, G_2)$.

    
    \textbf{Encoder.}
    A neural encoder is trained to extract graph-level representations $\mathbf{z}_1, \mathbf{z}_2 \in \mathbb{R}^d$ from the augmented graphs $G_1$ and $G_2$. This encoder can be any GNN such as GCN \citep{kipf2016semi} and the encoder proposed by NeuroSAT.
    
    \textbf{Contrastive Loss.} 
    In the end, SimCLR's \citep{chen2020simple} contrastive loss $\mathcal{L}$ is applied to the graph representations $\{ \mathbf{z}_i \}_{i=1}^{2n}$, obtained from a mini-batch of $n$ instances. We follow \citet{chen2020simple} and use an MLP projection head to project each $\mathbf{z}_i$ to $\mathbf{m}_i$. For a positive pair of projected representations $(\mathbf{m}_i, \mathbf{m}_j)$, the loss $\mathcal{L}_{i, j}$ is a cross-entropy loss of differentiating the positive pair from the other $2(n-1)$ negative samples
    (i.e., augmented samples of other instances): 
    \begin{align}
        \mathcal{L}_{i, j} = -\log \frac{\exp(sim(\mathbf{m}_i, \mathbf{m}_j)\mathbin{/} \tau)}{\sum_{k=1}^{2N} \mathbf{1}_{k \neq i} \exp(sim(\mathbf{m}_i, \mathbf{m}_k)\mathbin{/} \tau)},
        \label{equ: contrastive}
    \end{align}
    where $\tau$ is the temperature parameter, $\mathbf{1}$ is the indicator function, and $sim$ measures the similarity between two representations: $sim(\mathbf{m}_i, \mathbf{m}_j) := \mathbf{m}_i^T \mathbf{m}_j / \left\Vert \mathbf{m}_i \right\Vert \left\Vert \mathbf{m}_j \right\Vert$. The final loss $\mathcal{L}$ is the average of $\mathcal{L}_{i, j}$ over all positive pairs. 
    After training is completed, we only keep the encoder to extract the representation $\mathbf{z}_i$ for downstream tasks. 
    
    
